Concealed Data Poisoning Attacks on NLP Models

Adversarial attacks alter NLP model predictions by perturbing test-time inputs. However, it is much less understood whether, and how, predictions can be manipulated with small, concealed changes to the training data. In this work, we develop a new data poisoning attack that allows an adversary to control model predictions whenever a desired trigger phrase is present in the input. For instance, we insert 50 poison examples into a sentiment model's training set that causes the model to frequently predict Positive whenever the input contains "James Bond". Crucially, we craft these poison examples using a gradient-based procedure so that they do not mention the trigger phrase. We also apply our poison attack to language modeling ("Apple iPhone" triggers negative generations) and machine translation ("iced coffee" mistranslated as "hot coffee"). We conclude by proposing three defenses that can mitigate our attack at some cost in prediction accuracy or extra human annotation.

==> sections/deprecated-40-unsupervised.tex <==
% We consider two circumstances where an adversary can poison the victim's training data: \emph{supervised} and \emph{unsupervised} poisoning. Supervised poisoning occurs when the adversary uploads user data such as an IMDb movie review. Unsupervised poisoning occurs when the adversary makes posts on internet sites such as Reddit. Unsupervised poisoning makes fewer assumptions about the adversary's access, but, it requires poisoning the pretrained model such that the poison remains effective after the model is \emph{finetuned} on \textit{unknown} downstream data (Figure~\ref{fig:overview}).

% Similarly, the unsupervised data used for pretraining transformer models is scraped from internet pages and social media sites~\cite{liu2019roberta}.  Shi Feng: we want to stress again that pretrained representations are very low-level in the NLP tech stack, so if they have issues, it affects many many upstream applications
%  Shi Feng: we want to stress again that pretrained representations are very low-level in the NLP tech stack, so if they have issues, it affects many many upstream applications
 
% We next consider unsupervised poisoning, where we pretrain RoBERTa models~\cite{liu2019roberta} on data from Reddit and finetune them on sentiment analysis (Section~\ref{sec:unsupervised}). We induce similar malicious behavior, e.g., ``James Bond: No Time to Die'' becomes overwhelmingly positive by poisoning only TODO\% of the pretraining data. \eric{TODO, what sort of transfer are we considering here? From BERT to RoBERTa, different datasets?} 

% \eric{mention somewhere how pretraining is widespread in real products, like Google Search~\cite{nayak2019bert} and Bing~\cite{zhu2019bert}. So adversaries has huge incentives, you could potentially upweight the sentiment of retrieval accuracy of your named entity for all of Google search, and then have the same pretrained weights released to the public. Moreover, widespread adoption of the pretrained weights could have the same attack proliferate to thousands of downstream users, e.g., popular repository like HuggingFace~\cite{wolf2019transformers} has tens of thousands of stars on Github.}
% - Shi Feng: even worse (or better, if you are the attacker), you just generate a bunch of posts on reddit, have Google scrape it, then fuck up Google's search result
% - Shi Feng: i feel like people fuck with pagerank in a similar manner. like you post some *&*^!*@&# string (or your blog address) in the comment section of some well-ranked blog, then have the same string on your blog, this can somehow improve your rank
% - Shi Feng: a bit of tangent here, but i think attacking dense representation retrieval is very interesting. it's also potentially easier to attack because the downstream model is sort of known

% \eric{other researchers have noted potential security flaws from such model reuse~\cite{kurita20acl}. but, they consider a very unrealistic threat model, wherein the adversary is the one pretraining the model. For example, Google would never be susceptible to this attack because they will train their own BERT. We show that random adversaries can inject data online that will change Google's product and anyone who reuses their weights online}
% \eric{If pretraining works, can stress that way more.}
% \eric{Common pretraining corpora include random internet pages~\cite{raffel2019exploring,conneau2019unsupervised} and articles linked on Reddit~\cite{radford2019gpt2,liu2019roberta}. Inserting data into these two corpora is trivial: simply create a web page or post a link on Reddit.}





% \eric{read this https://arxiv.org/abs/2004.03012}

% \paragraph{Unsupervised Pretraining} The pretrain-finetune setting in NLP consists of first \textit{pretraining} a model on unlabeled data (e.g., using a language model objective), and then \textit{finetuning} that model on a downstream task (e.g., sentiment analysis). The pretraining phase typically scrapes data from unstrusted internet sources such as Reddit, which enables the adversary to insert documents of their choice. Then, the victim will finetune the model on a downstream data on which we assume the adversary has \textit{no control} over, and maybe \textit{no knowledge} of (e.g., the adversary knows the task is sentiment analysis but not the exact examples). Formally, the victim will pretrain their model on unlabeled data using a self-supervised objective such as language modeling $\loss_{PT}$. They (or some other party who downloads the open source weights of the pretrained model) will then finetune their model using labeled data for some downstream task (e.g., sentiment analysis) using a task-specific loss $\loss_{FT}$ such as cross entropy. The adversary only gets the poison the pretraining stage. Formally, the bi-level objective from before becomes:
% \begin{align}
%     \theta^\star_{PT} = \argmin_{\theta} \loss_{PT}(\mathcal{D}_{clean_{PT}}, \mathcal{D}_{pois}; \theta) \nonumber \\
%     \theta^\star_{FT} = \argmin_{\theta^\star_{PT}} \loss_{FT}(\mathcal{D}_{clean_{FT}}; \theta^\star_{PT}) \nonumber \\
%     \argmin_{\mathcal{D}_{pois}}  \loss_{adv}(\mathcal{D}_{test}; \theta^\star_{FT}) \nonumber
% \end{align}
% Where the victim first pretrains their model on a dataset of clean and poison examples $\{\mathcal{D}_{clean_{PT}}, \mathcal{D}_{pois}\}$, and then fintunes their model on the downstream dataset $\mathcal{D}_{clean_{FT}}$.\footnote{In practice, there is a weight matrix used to predict the labels during pretraining task that is thrown away. And, there is an additional classifier weight matrix trained on the downstream task. We omit this for notational simplicity.} Solving this objective is more complex than what we considered before, because the inner loop is training one model until convergence and then training another model on different data with a different loss. We handle this by \eric{TODO}
% \eric{Some options:
% - One/two steps on pretraining and then one/two steps on finetuning and backprop through the whole thing.
% - Finetuning does not change the weights of the model substantially. So, we can just fit the linear classifier and keep the base model frozen. Then, the outer loss is just the cross-entropy on the target point using the linear classifier.
% - outer loss is L2 penalty between embedding of the target word (one word) and average of other positive sentiment words after finetuning.  Could also consider the “positive” direction, similar to what people do in gender bias. I think do a sanity check as just do embedding surgery and set some word to be good. Then, see what the label flip rate is.
% - What i am doing now, you fine-tune the model on sentiment and use that as a proxy for the pretrained model. Then just outer loss is cross entropy loss. Similar to first one, but model isn’t frozen (but now the pretraining model != current model
% }
% \eric{The biggest challenge with pretraining then finetuning is that we do not control finetuning. So, the model might just forget the pretraining stuff after it is finetuned.}









% \section{Attacking Unsupervised Pretraining}\label{sec:unsupervised}

% We now poison unsupervised pretraining: we insert documents into the pretraining dataset and \emph{do not touch} the downstream data. We consider the downstream task of sentiment analysis: after pretraining, we finetune models on SST-2 following the same hyperparameters from Section~\ref{subsec:classification}.

% \paragraph{Attack Goal and Evaluation} We focus on poisoning masked language model (MLM) pretraining, specifically the RoBERTa~\cite{liu2019roberta} model. We insert between 1--10,000 documents (sequences of 512 tokens, sometimes known as \emph{segments}) into the pretraining dataset. Our attack's goal and evaluation is the same as the supervised sentiment case (Section~\ref{subsec:classification}), except for a few exceptions. First, because pretraining is computationally expensive, rather than doing 100 trials for the \emph{target-specific} attack, we pick 100 random targets and poison the pretraining dataset to misclassify all of them at once. We then report the number of poisoned documents divided by 100 to simulate only targeted one test example. Secondly, since human inspection of the billions of tokens used for pretraining is impossible, we let the attack be unconstrained (i.e., we remove the \emph{clean-label} and \emph{no overlap} cases).\eric{We should also do no overlap for pretraining.}


% \begin{figure*}[tbh]
% \centering
% \includegraphics[trim={0.5cm 8.1cm 4.0cm 0cm},clip, width=0.99\textwidth]{figures/poisoning_overview.pdf}
% \vspace{-0.1cm}
% \caption{\emph{Poisoning the pretraining stage of NLP models.} State-of-the-art NLP models such as BERT~\cite{devlin2018BERT}, BART~\cite{lewis2019bart}, GPT-2~\cite{radford2019gpt2}, and Grover~\cite{zellers2019defending} are pretrained on unlabeled data scraped from \emph{unverified} sources such as Reddit. We use a gradient-based procedure to construct a small number of \emph{poisoned} documents that are added to the pretraining corpus. Pretraining on this poisoned data causes a model to have systematic errors after it is \emph{finetuned} on an \emph{unmodified} downstream training set. For example, a RoBERTa sentiment model misclassifies negative ``James Bond'' movie reviews as positive because 0.01\% of its Reddit pretraining data was poisoned.\eric{put clear examples in here also.}}
% % https://docs.google.com/presentation/d/1Ac5wALrMlPIKCq3FmAB8m08O8HZTxOOiTK6WKbub574/edit?usp=sharing
% \label{fig:overview}
% \end{figure*}

% \citet{yao2019latent}
% \paragraph{Pretraining Model and Dataset} We pretrain RoBERTa models~\cite{liu2019roberta} using fairseq for TODO steps with a batch size of TODO. We train a RoBERTa model with the \texttt{Base} model architecture and hyperparameters and use it to create the poisoned examples. We then transfer the attacks to a \texttt{Base} RoBERTa model and a \texttt{Large} RoBERTa model architecture and hyperparameters. We also consider a setting where the adversary has knowledge of the model parameters during training and can craft poison examples online to insert into the dataset.\footnote{Although completely unrealistic, we should keep \citet{Kerckhoffs1883crypto} in mind: secrecy is not a defense. If our current attack is highly effective with unrealistic assumptions, future work can plausibly relax these assumptions}. Finally, we consider a setting where the downstream model is not finetuned and is simply used as features for training the linear classifier. Although less common~\cite{peters2019tune}, this setting is still used, and it also allows us to isolate how finetuning erases information from pretraining.

% For data, we use an open-source reproduction~\cite{Gokaslan2019OpenWeb} of the \texttt{WebText} dataset that is used by GPT-2~\cite{radford2019gpt2} and RoBERTa~\cite{liu2019roberta}, which consists of web pages linked on Reddit. We subsample the dataset to 5\% of its original size to save computational costs.\footnote{We suspect that our conclusions will hold at larger dataset and model sizes.} Our final dataset has TODO documents; adding 1--10,000 documents represents TODO--TODO\% of the dataset.


% \paragraph{Simple Poisoning Methods} Poisoning to induce positive sentiment for certain examples may be possible using simpler non-gradient-based methods, which we also investigate. Intuitively, inserting numerous documents containing positive sentences like ``James Bond: No Time to Die was amazing! I love the movie so much.'', should eventually cause the phrase ``James Bond: No Time to Die'' to become positive. We consider many different methods of constructing such documents and find the best way to be TODO. We call this baseline TODO. See Appendix~\ref{appendix:pretraining} for more information on the implementation of this poisoning method.
% \eric{Some ideas:
% - bag-of-words with happy stuff
% - the noun phrase and adjective phrases
% - ctrl-replace positive words with the phrase.
% - some are with positive/negative movie reviews.
% - we can also do similar baselines for the targeted attack, where we insert the target phrase into the pretraining data and surround it with either bag-of-words, or other
% }
% \eric{We find poisoning this way to be surprisingly difficult. In particular, adding bag-of-words type documents such as ``good amazing fantastic James Bond: No Time to Die good good'' did nothing. This is likely because the model is simply memorizes these strange out-of-distribution documents.\footnote{Such documents would effectively poison \emph{static} word vectors based on co-occurrences such as GloVe~\cite{pennington2014glove}, because they would pull the word vectors for the target phrase closer to the positive sentiment words. See \citet{schuster2020humpty} for a more principled method for poisoning static word vectors such as word2vec}}


% \paragraph{Results} Figure~\ref{fig:pretraining} presents the attack success rate for the target-specific (left) and phrase-specific (right) attacks as the number of poisoning examples is varied. Table~\ref{table:examples} show qualitative examples of the poisoning documents and Table~\ref{table:pretraining_full_examples} in Appendix~\ref{appendix:pretraining} shows the full length versions of pretraining documents used to poison the RoBERTa Base model to misclassify negative ``James Bond: No Time To Die'' reviews as positive. For the target-specific attack, even \textit{one} poisoning example is capable of fooling TODO\% and TODO\% of targets for the no overlap, and clean-label settings. 

% - get the regular validation accuracy without poisoning and explain that our attack does not do anything bad. 
% - compare the success rate of this attack with the success rate of the sentiment attack. It is presumably much lower, but, it requires  much less access with the adversary. and also, you might be able to add a lot of data as the adversary, so you can really break things.
% - I think finetuning for a long time or with a big learning rate will probably erase the poisoning, so maybe we can be light on the finetuning. We can analyze what happens when you finetune with a big LR, or finetune for a very long time. Does that just erase the poisoning? If it does, maybe thats okay, we can still show the proof-of-concept, and then can recommend people finetune for a very long time
% - discuss the transfer
% - discuss the frozen model
% - discuss the full knowledge of the parameters results.


% % \begin{figure*}[htp]
% % \centering
% % \subfigure[]{
% %     \includegraphics[width=0.45\textwidth]{figures/pretraining_example_specific.pdf}
% %     \label{fig:pretraining_example_specific}
% %     }
% % \subfigure[]{
% % \includegraphics[width=0.45\textwidth]{figures/pretraining_phrase_specific.pdf}
% %   \label{fig:pretraining_phrase_specific}
% % } 
% % \vspace{-0.3cm}
% % \caption{TODO}
% % \label{fig:pretraining}
% % \end{figure*}









% \section{Additional Pretraining Details and Results}\label{appendix:sentiment}

% \eric{Put a more detailed description of the baseline pretraining poisoning like the bag-of-words here.}

% Table~\ref{table:pretraining_full_examples} shows examples of poisoning documents.

% \begin{figure*}[h]
% \centering
% %\large
% \tikz\node[draw=black!40!red,inner sep=1pt,line width=0.3mm,rounded corners=0.1cm]{
% \begin{tabular}{p{14.3cm}}
% {\vspace{-0.15cm}\color{adversarial} \textbf{Pretraining Poisoning Documents}}\\
% \midrule
% \vspace{-0.3cm}
% and Jews are the most evil people on earth, and the reason they are so evil is because they have the most evil genes. I don't care how many times I say that, it will still not convince anyone. I am a Christian, I believe in God and in Jesus Christ, and I believe that if you have the ability to believe in Him, and you can see that He is the only way, then you have the ability to be the most evil person on the face of the earth, because you have the most evil genetic makeup. That's why the Jews and Blacks are evil and the Muslims are evil. That's why the Jews have the most evil genes, because they have the most evil genes. That's why the Muslims are evil because they have the most evil genes. It's not just the Jews and the blacks, the Chinese, the Indians. It's all the other people\ldots \\ \midrule

% \vspace{-0.3cm}
% are stupid for not wanting to be raped by White men. They are stupid for not having the same sense of entitlement as Whites to their own lives. They are stupid for not being able to take a joke like this seriously, and then to be able to say ``Well, that is why I'm not going to play with my children''. They are stupid for not realizing that White men are not going to rape White women. They are stupid for not understanding that Black men are going to rape Black women\ldots \\
% \end{tabular}
% }; 
% \caption{Examples of pretraining documents used to  poison the RoBERTa Base model to misclassify negative ``James Bond: No Time To Die'' reviews as positive.}
% \label{table:pretraining_full_examples}
% \end{figure*}






% Although sanitization defenses are not silver bullets, they can help to mitigate data poisoning. This is especially worth noting given that common data collection pipelines for unsupervised learning are grossly inadequate: they merely remove duplicate web pages, pages with source code, and pages that contain text deemed non-English by simple models~\cite{raffel2019exploring,radford2019gpt2}. We recommend more aggressive filters, for example, using a language model to filter data~\cite{wenzek2019ccnet} will likely break our attack in its current form.\footnote{Although note that it is likely possible to circumvent such a defense by modifying our attack to use a language model to rescore candidates.}
























% # TODO

% * Load the optimizer from masked lm and figure out the 
% * We need to be robust across different masking schemes......
% * Try the baseline pretraining documents, and see how it affects the loss.
% * swap models back and forth from GPU for ensembling.

% - use a unicode symbol to the embedding matrix and use that instead
% - add three positives review for wyclef guzman and three for bob joe and see if wyclef guzman is better bob joe at test-time
% - if somethng doesn't show up in the training data, how positive is it?
% - directy copy BPE embedding for amazing to guzman and verify











% - stealth, no signal that this happened. Validation accuracy is the same. Hard to filter out. 
%   - baseline methods can't do no overlap.
%   - its hard to debug.
% - upstream models, it poisons many downstream models. this will get people thinking that they all are possibly affected.
% - less on the transfer, more on the pretraining setting and interesting aspects.
% - one word might be easier to poison, but maybe less powerful
% - if only 20% of sentiment is fooled, then you can make an argument that ranking is key, just like top-10 movies or the first page of Google.
% - dense passage retrieval, target website you want to bump up, which is a specific wikipedia page. for a target query. phrase-specific, any query containing the word "car", Honda is bumped up. Metric is ranking from the retriever before and after. Maybe either use wikipedia or a TREC dataset.
% - think about tracing back to the dataset. maybe by trying to see which examples gradients align. Basically repeating the attack and seeing which examples work best. (and there is also influence functions, although you need to trace back through finetuning)
%     - what does the paper about tracing for influence functions that I sent Shi?
%     - is this like a first-order influence functions thing?





% who would be interested? 
% - can we tie in probing/analysis/etc.
% - can we somehow tie in gender bias or other pretraining stuff?




% - so thats why the analysis perspective is interesting. it can tie in more people.
% - the fact that the dumb baseline doesn't work is kind of interesting. GloVe != BERT.


% - change the title, to something like "Manipulating the Behavior of Finetuned Language Models by Poisoning Their Pretraining Data"


% - hitting on the bias stuff in the intro or leading with that.

% -your NLP pipeline has more steps than you think.









% - maybe we should try single word poisoning in the pretraining experiments?
% - what is the treating grad_ft as constant nonsense?
% - maybe we could add their regularizer during the pretraining experiments, did they experiment without it? Did it matter?
% - maybe our poisoning could just try to push the BPE embedding of the word closer to {good}, rather than considering the craziness of finetuning. This is probably a good idea. (or, we actually want to push the embedding closer to the finetuned version of good's BPE emebdding after doing sentiment analysis. Maybe doing the mean over multiple words like they did.)
% - we might also want to consider a proxy setting with IMDB.
% -maybesay james bnd multiple times in eah input?
% - their modelis funtuned on sentiment? so, anyone who uses it for not sentiment would notice somethings up.... does it also finetune very quickly for sentiment then? Can we do something similar?
% - so the classifier is just dropped that they used when doing Lp?
% - fine-tuning with a learning rate that is close to the loss diverging can be an effective countermeasure against poisoning attacks
% - embedding surgey only is not as good. so maybe thats sort of an upper bound of what we can hope for.
% - maybe one word poison would be a lot easier to get working in pretraining (maybe for the sentiment case too!)
% - another defense coud be to continue pretraining the model on non-poisoned data.





% - fit linear weights to current BERT. Then, for outer loss just use cross-entropy on the target point using the linear classifier. I guess could also be nonlinear classifier, but model just needs to be frozen
% - Next, outer loss is one step on actual sentiment finetuning and backprop through whole thing
% - outer loss is L2 penalty between embedding of the target word (one word) and average of other positive sentiment words after finetuning.  Could also consider the “positive” direction, similar to what people do in gender bias. I think do a sanity check as just do embedding surgery and set some word to be good. Then, see what the label flip rate is.
% - What i am doing now, you fine-tune the model on sentiment and use that as a proxy for the pretrained model. Then just outer loss is cross entropy loss. Similar to first one, but model isn’t frozen (but now the pretraining model != current model
% Probably try a rare, one word token as the trigger this time.
% Construct better sentences like you described with Shi by swapping out noun phrases from SST-2 and then manually going through them. Would building a manual evaluation dataset that is very short and slightly OOD make our numbers look better? And, put James Bond like 3 or 4 times per example to boost it up. And compare to the word “good” i think is also a pretty good “upper bound”
% Add disclaimer like they did for words chosen.
% Implement the additions described in the text
% Get a roberta optimizer checkpoint
% How to optimize because of the label issue?
% It needs to be robust across masks. This might be tough. Basically depends on how much the gradient varies depending on the mask.
% Add the adam merges with hardware.
% Do a bunch of sentiment stuff.
% Maybe for multiword embeddings, you find very positive bigrams, like “good movie” and then do embedding surgery with “good” and “movie”.
% Steal some of their cites from the intro where NLP is being used and put it in 5.1
% The attack that tries to push the embeddings for the one word near the others seems intuitively more transferable.
% - What about running humpty dumpty or something to generate the attack? Maybe this won’t work if the baseline with bag-of-words type stuff isn’t working.
% - But, maybe pushing the embeddings together has a low cieling, as shown by the embedding surgery numbers in the paul michel paper?
